Distributing circuits over heterogeneous, modular quantum computing network architectures

We consider a heterogeneous network of quantum computing modules, sparsely connected via Bell states. Operations across these connections constitute a computational bottleneck and they are likely to add more noise to the computation than operations performed within a module. We introduce several techniques for transforming a given quantum circuit into one implementable on a network of the aforementioned type, minimising the number of Bell states required to do so. We extend previous works on circuit distribution over fully connected networks to the case of heterogeneous networks. On the one hand, we extend the hypergraph approach of [Andres-Martinez & Heunen. 2019] to arbitrary network topologies. We additionally make use of Steiner trees to find efficient realisations of the entanglement sharing within the network, reusing already established connections as often as possible. On the other hand, we extend the embedding techniques of [Wu, et al. 2022] to networks with more than two modules. Furthermore, we discuss how these two seemingly incompatible approaches can be made to cooperate. Our proposal is implemented and benchmarked; the results confirming that, when orchestrated, the two approaches complement each other's weaknesses.

==> images/ALAP/input.tex <==

\begin{quantikz}[column sep=3mm]
    \lstick[1]{\texttt{A}} & \ctrl{2} &[-2.5pt] \dH{} & \ctrl{1} & \dH{} &[-2.5pt] \ctrl{2} & \qw \\[3pt]
    \lstick[1]{\texttt{B}} & \qw & \qw & \ctrl{} & \qw & \qw & \qw \\[-10pt]
    & \dPhase{\alpha} & & & & \dPhase{\beta} & \\[-10pt]
    \lstick[1]{\texttt{C}} & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw \\[3pt]
    \lstick[1]{\texttt{D}} & \qw & \qw & \qw & \qw & \ctrl{-2} & \qw  
\end{quantikz}

==> images/ALAP/right.tex <==

\begin{quantikz}[column sep=3mm]
    \lstick[1]{\texttt{A}} & \qw \arrow[d, squiggly] &[-3pt] \qw &[-3pt] \qw &[-3pt] \qw & \dH{} &[-2.5pt] \ctrl{2} &[-2.5pt] \qw &[-2.5pt] \dH{} & \qw &[-3pt] \qw &[-3pt] \qw &[-3pt] \qw & \qw \\[10pt]
    \lstick[2]{\texttt{B}} & & \qw \arrow[dd, squiggly] & \qw & \qw & \dH{} & \qw & \ctrl{1} & \dH{} & \qw \arrow[ddddd, squiggly] & \qw & \qw & \qw \arrow[u, squiggly] & \\
    \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{} & \ctrl{} & \qw & \qw & \qw & \qw & \qw & \qw \\[10pt]
    \lstick[3]{\texttt{C}} & & & \ctrl{1} & \qw \arrow[uu, squiggly] & & & & & & & & & \\[-10pt]
    & & & \dPhase{\alpha} & & & & & & & & & & \\[-10pt]
    \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \\[10pt]
    \lstick[3]{\texttt{D}} & & & & & & & & & & \ctrl{1} & \qw \arrow[uuuuu, squiggly] & & \\[-10pt]
    & & & & & & & & & & \dPhase{\beta} & & & \\[-10pt]
    \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw 
\end{quantikz}

==> images/ALAP/wrong.tex <==

\begin{quantikz}[column sep=3mm]
    \lstick[1]{\texttt{A}} & \qw \arrow[d, squiggly] &[-3pt] \qw & \qw &[-2.5pt] \dH{} &[-2.5pt] \ctrl{2} &[-2.5pt] \qw &[-3.5pt] \dH{} &[-2.5pt] \qw &[-2.5pt] \qw &[-2.5pt] \qw &[-6pt] \qw &[-3pt] \qw & \qw \\[10pt]
    \lstick[2]{\texttt{B}} & & \qw \arrow[ddddd, squiggly] & \qw \arrow[dd, squiggly] & \dH{} & \qw & \ctrl{1} & \dH{} & \qw & \qw & \qw & \qw & \qw \arrow[u, squiggly] & \\
    \qw & \qw & \qw & \qw & \qw & \ctrl{} & \ctrl{} & \control[red]{} \arrow[d, dash, thick, red] & \control[red]{} \arrow[dddd, dash, thick, red] & \qw & \qw & \qw & \qw & \qw \\[10pt]
    \lstick[3]{\texttt{C}} & & & & \ctrl{1} & \qw & \dH{} & \control[red]{} & \qw & \dH{} & \qw \arrow[uu, squiggly] & & & \\[-10pt]
    & & & & \dPhase{\alpha} & & & & & & & & & \\[-10pt]
    \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \\[10pt]
    \lstick[3]{\texttt{D}} & & & \qw & \qw & \qw & \dH{} & \qw & \control[red]{} & \dH{} & \ctrl{1} & \qw \arrow[uuuuu, squiggly] & & \\[-10pt]
    & & & & & & & & & & \dPhase{\beta} & & & \\[-10pt]
    \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw 
\end{quantikz}

==> images/embedding_conflict/a.tex <==

\begin{quantikz}[column sep=3mm]
    \lstick[1]{\texttt{A}} & \dHblue{} & \ctrl{} \arrow[d, dash, thick, "x"] & \dHblue{} & \qw \\[5pt]
    \lstick[1]{\texttt{B}} & \dHorange{} & \ctrl{} & \dHorange{} & \qw
\end{quantikz}

==> images/embedding_conflict/b.tex <==

\begin{quantikz}[column sep=3mm]
  \lstick[1]{\texttt{A}} & \qw \arrow[d, squiggly] & \dHblue{} & \ctrl{} \arrow[dd, dash, thick, "x" yshift=3mm] & \qw & \dHblue{} & \qw & \qw \\[5pt]
  \lstick[2]{\texttt{B}} & & \dHblue{} & \qw & \ctrl{} \arrow[d, dash, thick, "y"] & \dHblue{} & \qw \arrow[u, squiggly] & \\[-5pt]
  \qw & \qw & \dHorange{} & \ctrl{} & \ctrl{} & \dHorange{} & \qw & \qw & 
\end{quantikz}

==> images/embedding_conflict/c.tex <==

\begin{quantikz}[column sep=3mm]
  \lstick[2]{\texttt{A}} & \qw &[5pt] \qw \arrow[dd, squiggly] &[3pt] \dHblue{} & \ctrl{} \arrow[ddd, dash, thick, "x"] & \ctrl{} \arrow[d, dash, thick, "x'"] & \qw & \qw & \dHblue{} &[3pt] \qw &[5pt] \qw & \qw \\[-5pt]
   & & \qw & \dHorange{} & \qw & \ctrl{}  & \qw & \control[red]{} \arrow[d, dash, thick, red, "y'"] & \dHorange{} & \qw & \qw \arrow[dd, squiggly] & \\[5pt]
  \lstick[2]{\texttt{B}} & & & \dHblue{} & \qw & \qw & \ctrl{} \arrow[d, dash, thick, "y"] & \control[red]{} & \dHblue{} & \qw \arrow[uu, squiggly] & & \\[-5pt]
  \qw & \qw \arrow[uu, squiggly] & \qw & \dHorange{} & \ctrl{} & \qw & \ctrl{} & \qw & \dHorange{} & \qw & \qw & \qw 
\end{quantikz}

==> images/embedding_example/HCZH.tex <==

\begin{quantikz}[column sep=3mm]
  \lstick[1]{\texttt{A}} &[-3pt] \ctrl{1} &[-3pt] \dH{} & \ctrl{} \arrow[ddd, dash, thick, "x"] & \dH{} &[-3pt] \ctrl{1} &[-3pt] \qw \\[-3pt]
   & \dPhase{\alpha} & & & & \dPhase{\beta} & \\[-3pt]
  \lstick[3]{\texttt{B}} & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw \\[-10pt]
  \qw & \qw & \qw & \ctrl{} & \qw & \qw & \qw \\[-10pt]
  \qw & \qw & \qw & \qw & \qw & \ctrl{-3} & \qw 
\end{quantikz}

==> images/embedding_example/HCZH_emb.tex <==

\begin{quantikz}[column sep=3mm]
  \qw & \qw \arrow[d, squiggly] &[-3pt] \qw &[-3pt] \dH{} & \ctrl{} \arrow[dddd, dash, thick, "x" yshift=-11pt] & \qw & \dH{} &[-3pt] \qw &[-3pt] \qw & \qw \rstick[1]{\texttt{A}} \\[8pt]
  & & \ctrl{1} & \dH{} & \qw & \ctrl{} \arrow[ddd, dash, thick, "x'" yshift=4pt] & \dH{} & \ctrl{1} & \qw \arrow[u, squiggly] & \rstick[5]{\texttt{B}} \\[-11pt]
  & & \dPhase{\alpha} & & & & & \dPhase{\beta} & & \\[-10pt]
  \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw \\[-10pt]
  \qw & \qw & \qw & \qw & \ctrl{} & \ctrl{} & \qw & \qw & \qw & \qw \\[-10pt]
  \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-3} & \qw & \qw
\end{quantikz}

==> images/embedding_example/HZH.tex <==

\begin{quantikz}[column sep=3mm]
  \lstick[1]{\texttt{A}} & \ctrl{1} & \dH{} &[-3pt] \dRz{\pi} &[-3pt] \dH{} & \ctrl{1} & \qw \\[-10pt]
  & \dPhase{\alpha} & & & & \dPhase{\beta} & \\[-7pt]
  \lstick[2]{\texttt{B}} & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw \\[-10pt]
  \qw & \qw & \qw & \qw & \qw & \ctrl{-2} & \qw
\end{quantikz}

==> images/embedding_example/HZH_emb.tex <==

\begin{quantikz}[column sep=3mm]
  \qw & \qw \arrow[d, squiggly] &[-3pt] \qw &[-3pt] \dH{} &[-3pt] \dRz{\pi} &[-3pt] \dH{} &[-3pt] \qw &[-3pt] \qw & \qw \rstick[1]{\texttt{A}} \\[5pt]
  & & \ctrl{1} & \dH{} & \dRz{\pi} & \dH{} & \ctrl{1} & \qw \arrow[u, squiggly] & \rstick[4]{\texttt{B}} \\[-13pt]
  & & \dPhase{\alpha} & & & & \dPhase{\beta} & & \\[-10pt]
  \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \qw \\[-10pt]
  \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-2} & \qw & \qw \\[-10pt]
\end{quantikz}

==> images/intertwined/final.tex <==

\begin{quantikz}[column sep=2mm]
    \lstick{\texttt{A}} & \qw \arrow[d, squiggly] & \qw & \dH{} & \qw \arrow[dd, squiggly] & \qw & \qw & \dH{} & \qw & \qw & \dH{} & \qw & \qw & \qw \\
    \lstick[4]{\texttt{B}} & & \ctrl{1} & \dH{} & \qw & \ctrl{1} & \qw & \dH{} & \ctrl{} \arrow[ddd, dash, thick, "y" yshift=10pt] & \qw \arrow[u, squiggly] & & & & \\
     & & \dPhase{\alpha} & & & \targ{} & \ctrl{} \arrow[dd, dash, thick, "x"] & \dH{} & \qw & \ctrl{} \arrow[dd, dash, thick, "y'"] & \dH{} & \ctrl{1} & \qw \arrow[uu, squiggly] & \\[-13pt]
     & & & & & & & & & & & \dPhase{\beta} & & \\[-10pt]
    \qw & \qw & \ctrl{-2} & \dDots{} & \qw & \qw & \ctrl{} & \dDots{} & \ctrl{} & \ctrl{} & \dDots{} & \ctrl{-1} & \qw & \qw 
\end{quantikz}

==> images/intertwined/input.tex <==

\begin{quantikz}[column sep=2mm]
    \lstick{\texttt{A}} &[-3pt] \ctrl{1} &[-3pt] \dH{} & \ctrl{} \arrow[dd, dash, thick, "x"] & \dH{} & \ctrl{} \arrow[dd, dash, thick, "y"] & \dH{} &[-3pt] \ctrl{1} &[-3pt] \qw \\[-10pt]
     & \dPhase{\alpha} & & & & & & \dPhase{\beta} & \\[-10pt]
    \lstick{\texttt{B}} & \ctrl{-1} & \dDots{} & \ctrl{} & \dDots{} & \ctrl{} & \dDots{} & \ctrl{-1} & \qw 
\end{quantikz}

==> images/intertwined/intermediate.tex <==

\begin{quantikz}[column sep=2mm]
    \lstick{\texttt{A}} &[-3pt] \ctrl{1} &[-3pt] \dH{} & \qw \arrow[d, squiggly] & \qw & \dH{} & \ctrl{} \arrow[ddd, dash, thick, "y" yshift=12pt] & \qw & \dH{} &[-3pt] \qw &[-3pt] \qw & \qw \\
    \lstick[3]{\texttt{B}} & \dPhase{\alpha} & & & \ctrl{} \arrow[dd, dash, thick, "x"] & \dH{} & \qw & \ctrl{} \arrow[dd, dash, thick, "y'"] & \dH{} & \ctrl{1} & \qw \arrow[u, squiggly] & \\[-13pt]
     & & & & & & & & & \dPhase{\beta} & & \\[-10pt]
    \qw & \ctrl{-2} & \dDots{} & \qw & \ctrl{} & \dDots{} & \ctrl{} & \ctrl{} & \dDots{} & \ctrl{-1} & \qw & \qw
\end{quantikz}

==> images/justifying_hypergraphs/dist.tex <==

\begin{quantikz}[column sep=3mm]
    \lstick[5]{\texttt{A}} &[5pt] \lstick[1]{\small $q_0$} & \qw & \ctrl{1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \\[-10pt]
    & & & \dPhase{\alpha} & & & & & & & & & \\[-10pt]
    & \lstick[1]{\small $q_1$} & \qw & \qw & \ctrl{1} & \qw & \qw & \dH{} & \qw \arrow[ddd, squiggly, thin] & \qw & \qw & \qw & \qw \\[-10pt]
    & & & & \dPhase{\beta} & & & & & & & & \\[-10pt]
    & & & \ctrl{-3} & \ctrl{-1} & \qw \arrow[ddd, squiggly, thin] & & & & & & & \\[10pt]
    \lstick[5]{\texttt{B}} & & & & & & & & & \ctrl{1} & \ctrl{3} & \qw \arrow[uuu, squiggly, thin] & \\[-10pt]
    & & & & & & & & & \dPhase{\delta} & & & \\[-10pt]
    & \lstick[1]{\small $q_2$} & \qw \arrow[uuu, squiggly, thin] & \qw & \qw & \qw & \dH{} & \ctrl{1} & \dH{} & \ctrl{-1} & \qw & \qw & \qw \\[-10pt]
    & & & & & & & \dPhase{\gamma} & & & \dPhase{\epsilon} & & \\[-10pt]
    & \lstick[1]{\small $q_3$} & \qw & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \dH{} & \ctrl{-1} & \qw & \qw 
\end{quantikz}

==> images/justifying_hypergraphs/graph.tex <==

\begin{tikzpicture}
  \node[circle, draw=black, fill=white, inner sep=1pt] (A) at (135:20mm) {\large $q_0$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (B) at (45:20mm) {\large $q_1$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (C) at (225:20mm) {\large $q_2$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (D) at (315:20mm) {\large $q_3$};
  \draw[thick] (A) -- node[left] {$\alpha$} (C);
  \draw[thick] (B) to[in=60, out=210, looseness=0.75] node[above left] {$\beta$} (C);
  \draw[thick] (C) -- node[below] {$\gamma$} (D);
  \draw[thick] (B) to[in=30, out=240, looseness=0.75] node[below right] {$\delta$} (C);
  \draw[thick] (B) -- node[right] {$\epsilon$} (D);
\end{tikzpicture}

==> images/justifying_hypergraphs/hyp.tex <==

\begin{tikzpicture}
  \coordinate (auxC) at (135:5mm);
  \coordinate (auxB) at (325:7mm);
  \node[circle, draw=black, fill=white, inner sep=1pt] (A) at (135:25mm) {\large $q_0$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (B) at (45:25mm) {\large $q_1$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (C) at (225:25mm) {\large $q_2$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (D) at (315:25mm) {\large $q_3$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (a) at (140:14.5mm) {$\alpha$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (b) at (70:10mm) {$\beta$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (c) at (270:17.5mm) {$\gamma$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (d) at (240:11mm) {$\delta$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (e) at (315:14mm) {$\epsilon$};
  \draw[thick] (auxC) -- (C);
  \draw[thick] (auxC) -- (a);
  \draw[thick] (auxC) -- (b);
  \draw[thick] (auxB) -- (B);
  \draw[thick] (auxB) -- (d);
  \draw[thick] (auxB) -- (e);
  \draw[thick] (C) -- (d);
  \draw[thick] (D) -- (e);
  \draw[thick] (B) -- (b);
  \draw[thick] (A) -- (a);
  \draw[thick] (D) -- (c);
  \draw[thick] (C) -- (c);
\end{tikzpicture}

==> images/justifying_hypergraphs/input_circuit.tex <==

\begin{quantikz}[column sep=4mm]
    \lstick[1]{\small $q_0$} &[-2.5pt] \ctrl{1} &[-5pt] \qw &[-2.5pt] \qw &[-2.5pt] \qw &[-2.5pt] \qw &[-2.5pt] \qw &[-5pt] \qw &[-2.5pt] \qw \\[-7pt]
    & \dPhase{\alpha} & & & & & & & \\[-7pt]
    \lstick[1]{\small $q_1$} & \qw & \ctrl{1} & \qw & \dH{} & \qw & \ctrl{1} & \ctrl{3} & \qw \\[-7pt]
    & & \dPhase{\beta} & & & & \dPhase{\delta} & & \\[-7pt]
    \lstick[1]{\small $q_2$} & \ctrl{-3} & \ctrl{-1} & \dH{} & \ctrl{1} & \dH{} & \ctrl{-1} & \qw & \qw \\[-7pt]
    & & & & \dPhase{\gamma} & & & \dPhase{\epsilon} & \\[-7pt]
    \lstick[1]{\small $q_3$} & \qw & \qw & \qw & \ctrl{-1} & \qw & \dH{} & \ctrl{-1} & \qw 
\end{quantikz}

==> images/justifying_hypergraphs/partition.tex <==

\begin{tikzpicture}
  \coordinate (auxC) at (135:5mm);
  \coordinate (auxB) at (325:7mm);
  \node[circle, draw=black, fill=white, inner sep=1pt] (A) at (135:25mm) {\large $q_0$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (B) at (45:25mm) {\large $q_1$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (C) at (225:25mm) {\large $q_2$};
  \node[circle, draw=black, fill=white, inner sep=1pt] (D) at (315:25mm) {\large $q_3$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (a) at (140:14.5mm) {$\alpha$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (b) at (70:10mm) {$\beta$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (c) at (270:17.5mm) {$\gamma$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (d) at (240:11mm) {$\delta$};
  \node[circle, draw=black, fill=white, inner sep=1pt, minimum size=5mm] (e) at (315:14mm) {$\epsilon$};
  \draw[thick] (auxC) -- (C);
  \draw[thick] (auxC) -- (a);
  \draw[thick] (auxC) -- (b);
  \draw[thick] (auxB) -- (B);
  \draw[thick] (auxB) -- (d);
  \draw[thick] (auxB) -- (e);
  \draw[thick] (C) -- (d);
  \draw[thick] (D) -- (e);
  \draw[thick] (B) -- (b);
  \draw[thick] (A) -- (a);
  \draw[thick] (D) -- (c);
  \draw[thick] (C) -- (c);
  \coordinate (start) at (195:27mm);
  \coordinate (end) at (15:32mm);
  \draw[dashed, very thick, gray] (start) to[out=0, in=180] (end);
  \node[above right=5mm of start] (A) {\color{gray} \Large \texttt{A}};
  \node[below left=5mm of end] (B) {\color{gray} \Large \texttt{B}};
\end{tikzpicture}

==> images/steiner/T.tex <==
\begin{tikzpicture}
    \node (net) {
        \begin{tikzpicture}
            \node[draw, circle, thin, minimum size=1.2em, inner sep=2pt] (A) {\texttt{A}};
            \node[below=5mm of A, draw, circle, thin, minimum size=1.2em, inner sep=2pt] (D) {\texttt{D}};            
            \node[left=5mm of D, draw, circle, thin, minimum size=1.2em, inner sep=2pt] (B) {\texttt{B}};
            \node[below=5mm of D, draw, circle, thin, minimum size=1.2em, inner sep=2pt] (C) {\texttt{C}};
            \draw[thick] (A) -- (D);
            \draw[thick] (D) -- (B);
            \draw[thick] (D) -- (C);
        \end{tikzpicture}
    };
    \node[right=5mm of net] (circ) {
        \begin{quantikz}[column sep=3mm]
            \lstick[1]{\texttt{A}} & \qw \arrow[d, squiggly] & \qw & \qw & \qw & \qw & \qw & \qw & \qw \\[10pt]
            \lstick[1]{\texttt{D}} & & \qw \arrow[dddd, squiggly] & \qw \arrow[d, squiggly] & \qw & \qw & \qw & \qw \arrow[u, squiggly] & \\[10pt]
            \lstick[3]{\texttt{B}} & & & & \ctrl{1} & \qw \arrow[u, squiggly] & & & \\[-10pt]
            & & & & \dPhase{\alpha} & & & & \\[-10pt]
            \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw \\[10pt]
            \lstick[3]{\texttt{C}} & & & \qw & \ctrl{1} & \qw & \qw \arrow[uuuu, squiggly] & & \\[-10pt]
             & & & & \dPhase{\beta} & & & & \\[-10pt]
            \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw
        \end{quantikz}
    };
\end{tikzpicture}

==> images/steiner/input.tex <==
\begin{quantikz}[column sep=3mm]
    \lstick[1]{\texttt{A}} & \ctrl{1} & \ctrl{3} & \qw \\[-5pt]
     & \dPhase{\alpha} & & \\[-5pt]
    \lstick[1]{\texttt{B}} & \ctrl{-1} & \qw & \qw \\[-5pt]
      & & \dPhase{\beta} & \\[-5pt]
    \lstick[1]{\texttt{C}} & \qw & \ctrl{-1} & \qw 
\end{quantikz}

==> images/steiner/line.tex <==
\begin{tikzpicture}
    \node (net) {
        \begin{tikzpicture}
            \node[draw, circle, thin, minimum size=1.2em, inner sep=2pt] (A) {\texttt{A}};
            \node[below=5mm of A, draw, circle, thin, minimum size=1.2em, inner sep=2pt] (B) {\texttt{B}};
            \node[below=5mm of B, draw, circle, thin, minimum size=1.2em, inner sep=2pt] (C) {\texttt{C}};
            \draw[thick] (A) -- (B);
            \draw[thick] (B) -- (C);
        \end{tikzpicture}
    };
    \node[right=5mm of net] (circ) {
        \begin{quantikz}[column sep=3mm]
            \lstick[1]{\texttt{A}} & \qw \arrow[d, squiggly] & \qw & \qw & \qw & \qw & \qw \\[10pt]
            \lstick[3]{\texttt{B}} & & \qw \arrow[ddd, squiggly] & \ctrl{1} & \qw & \qw \arrow[u, squiggly] & \\[-10pt]
             & & & \dPhase{\alpha} & & & \\[-10pt]
            \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw \\[10pt]
            \lstick[3]{\texttt{C}} & & & \ctrl{1} & \qw \arrow[uuu, squiggly] & & \\[-10pt]
             & & & \dPhase{\beta} & & & \\[-10pt]
            \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw
        \end{quantikz}
    };
\end{tikzpicture}
